Capacity Bounds on the Downlink of Symmetric, Multi-Relay, Single Receiver C-RAN Networks

The downlink of symmetric Cloud Radio Access Networks (C-RANs) with multiple relays and a single receiver is studied. Lower and upper bounds are derived on the capacity. The lower bound is achieved by Marton's coding which facilitates dependence among the multiple-access channel inputs. The upper bound uses Ozarow's technique to augment the system with an auxiliary random variable. The bounds are studied over scalar Gaussian C-RANs and are shown to meet and characterize the capacity for interesting regimes of operation.

==> GaussianN3P1.tex <==

\begin{tikzpicture}[scale=.82]
  \begin{axis}[scale=.75,
width=4.82222222222222in,
%width=0.75\columnwidth,
height=3.80333333333333in,
scale only axis,
font=\normalsize,
xmin=0,
xmax=2,
%xmajorgrids,
xlabel={Link Capacity $C$},
ymin=0,
ymax=1.7,
%ymajorgrids,
ylabel={Rate $R$},
axis x line*=bottom,
axis y line*=left,
%legend pos=south east,
legend style={at={(.45,.1)},anchor=south west,legend cell align=left, font=\normalsize}
]
   
   
    \addplot[color=red,solid,line width=1.0pt,]
 table[row sep=crcr]{
              0         0\\
    0.0500    0.1500\\
    0.1000    0.3000\\
    0.1500    0.4500\\
    0.2000    0.6000\\
    0.2500    0.7500\\
    0.3000    0.9000\\
    0.3500    1.0499\\
    0.4000    1.1552\\
    0.4500    1.2284\\
    0.5000    1.2891\\
    0.5500    1.3384\\
    0.6000    1.3792\\
    0.6500    1.4135\\
    0.7000    1.4428\\
    0.7500    1.4681\\
    0.8000    1.4898\\
    0.8500    1.5093\\
    0.9000    1.5257\\
    0.9500    1.5407\\
    1.0000    1.5543\\
    1.0500    1.5668\\
    1.1000    1.5781\\
    1.1500    1.5888\\
    1.2000    1.5990\\
    1.2500    1.6081\\
    1.3000    1.6167\\
    1.3500    1.6242\\
    1.4000    1.6313\\
    1.4500    1.6379\\
    1.5000    1.6440\\
    1.5500    1.6487\\
    1.6000    1.6548\\
    1.6500    1.6595\\
    1.7000    1.6602\\
    1.7500    1.6604\\
    1.8000    1.6607\\
    1.8500    1.6604\\
    1.9000    1.6602\\
    1.9500    1.6600\\
    2.0000    1.6603     \\   };
    \addlegendentry{Upper bound of Theorem \ref{cor-up-Gaussian}}
    
      \addplot[color=blue,solid,line width=1.0pt,]
 table[row sep=crcr]{
         0         0\\
    0.0500    0.1500\\
    0.1000    0.3000\\
    0.1500    0.4500\\
    0.2000    0.6000\\
    0.2500    0.7500\\
    0.3000    0.9000\\
    0.3500    1.0459\\
    0.4000    1.1512\\
    0.4500    1.2284\\
    0.5000    1.2891\\
    0.5500    1.3384\\
    0.6000    1.3792\\
    0.6500    1.4135\\
    0.7000    1.4428\\
    0.7500    1.4681\\
    0.8000    1.4898\\
    0.8500    1.5093\\
    0.9000    1.5257\\
    0.9500    1.5407\\
    1.0000    1.5533\\
    1.0500    1.5648\\
    1.1000    1.5751\\
    1.1500    1.5838\\
    1.2000    1.5920\\
    1.2500    1.5991\\
    1.3000    1.6057\\
    1.3500    1.6112\\
    1.4000    1.6163\\
    1.4500    1.6209\\
    1.5000    1.6250\\
    1.5500    1.6287\\
    1.6000    1.6318\\
    1.6500    1.6345\\
    1.7000    1.6372\\
    1.7500    1.6394\\
    1.8000    1.6417\\
    1.8500    1.6434\\
    1.9000    1.6452\\
    1.9500    1.6470\\
    2.0000    1.6483\\
              };
    \addlegendentry{Lower bound of Theorem \ref{cor:lb-Gaussian}}
    \addplot[color=black,dotted,line width=1pt,]
 table[row sep=crcr]{
                       0.4508   0\\
                       0.4508 1.7\\
                       };
\addplot[color=black,dotted,line width=1pt,]
 table[row sep=crcr]{
                       0.8858   0\\
                       0.8858 1.7\\
                       };

\addplot[color=black,dotted,line width=1pt,]
 table[row sep=crcr]{
                       0.3333   0\\
                       0.3333 1.7\\
                       };
\addplot[color=black,dotted,line width=1pt,]
 table[row sep=crcr]{
                       1.6610   0\\
                       1.6610 1.7\\
                       };    
\draw[fill] (axis cs:{0.4508,0}) circle [radius=3pt] node[above right,yshift=.1cm] {$C_L$};
\draw[fill] (axis cs:{0.8858,0}) circle [radius=3pt] node[above right,yshift=.1cm] {$C_U$};
\draw[fill] (axis cs:{0.3333,0}) circle [radius=3pt] node[above left,yshift=.1cm] {$C_C$};
\draw[fill] (axis cs:{1.6610,0}) circle [radius=3pt] node[above right,yshift=.1cm] {$C_{\text{coop}}$};
\node[label=below:\rotatebox{90}{No Cooperation}] at (.15,1.26) {};
\node[label=below:\rotatebox{90}{Marton's Coding}] at (.675,1.26) {};
\node[label=below:\rotatebox{90}{Full Cooperation}] at (1.8,1.26) {};
    \end{axis}
    \end{tikzpicture}

